Probabilistic Interactive 3D Segmentation with Hierarchical Neural Processes

Interactive 3D segmentation has emerged as a promising solution for generating accurate object masks in complex 3D scenes by incorporating user-provided clicks. However, two critical challenges remain underexplored: (1) effectively generalizing from sparse user clicks to produce accurate segmentation, and (2) quantifying predictive uncertainty to help users identify unreliable regions. In this work, we propose NPISeg3D, a novel probabilistic framework that builds upon Neural Processes (NPs) to address these challenges. Specifically, NPISeg3D introduces a hierarchical latent variable structure with scene-specific and object-specific latent variables to enhance few-shot generalization by capturing both global context and object-specific characteristics. Additionally, we design a probabilistic prototype modulator that adaptively modulates click prototypes with object-specific latent variables, improving the model's ability to capture object-aware context and quantify predictive uncertainty. Experiments on four 3D point cloud datasets demonstrate that NPISeg3D achieves superior segmentation performance with fewer clicks while providing reliable uncertainty estimations.

==> table/partnet_main.tex <==
\begin{table}[!ht]
\centering
\setlength{\tabcolsep}{3pt}
\resizebox{0.98\linewidth}{!}{
\begin{tabular}{l|cc|cc}
\toprule
\textbf{Methods} & \textbf{IoU\myfavoriteat5} $\uparrow$ & \textbf{IoU\myfavoriteat10} $\uparrow$ & \textbf{NoC\myfavoriteat80} $\downarrow$ & \textbf{NoC\myfavoriteat85} $\downarrow$ \\
\midrule
InterObject3D  & 61.9 & 70.2 & 14.5 & 16.7 \\
InterObject3D++  & 60.0 & 70.8 & 13.9 & 16.4 \\
AGILE3D  & 59.6 & 70.1 & 14.5 & 16.7 \\
\rowcolor[gray]{.9} \textbf{NPISeg3D} & \textbf{63.2} & \textbf{73.2} & \textbf{13.0} & \textbf{15.2} \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Quantitative results on multi-part segmentation task on the PartNet dataset.} All models are required to predict multiple part masks simultaneously in a single scene. The model is trained on ScanNet40, and the best results are highlighted in \textbf{bold}.}
\label{tab:partnet_main}
\vspace{-4mm}
\end{table}
